CoDistill-GRPO: A Co-Distillation Recipe for Efficient Group Relative Policy Optimization

Group Relative Policy Optimization (GRPO) has emerged as a powerful algorithm for improving the reasoning capabilities of language models, but often fails to improve small models due to sparse rewards on difficult tasks. Existing works mitigate this issue by leveraging a larger model, either to provide hints for rollouts or to provide dense reward signals through knowledge distillation (KD). However, this assumes the existence of such an oracle, and training one can significantly increase total training time. In this work, we propose CoDistill-GRPO, a co-distillation algorithm that simultaneously trains a large and a small model by maximizing carefully designed GRPO objectives. The two models learn from each other: the small model uses an on-policy KD reward to learn from the large model's distribution, while the large model is updated using rollouts generated by the small model with importance reweighting, reducing the computational overhead of rollout generation. We show that CoDistill-GRPO substantially improves small model performance over standard GRPO on mathematical benchmarks across both Qwen and Llama models. Specifically, with Qwen2.5-Math-1.5B, we observe an accuracy increase of over 11.6 percentage points over the base model and an additional 6.0 percentage points over GRPO on the Minerva dataset. Interestingly, the larger model (Qwen2.5-Math-7B) trained with CoDistill-GRPO nearly matches standard GRPO performance despite training on small-model rollouts. This highlights CoDistill-GRPO as a cost-effective alternative to GRPO for larger models, yielding an approximate 18% speedup, which may be of independent interest.

==> temp.tex <==

\begin{proof}
    Recall that the reward $\widetilde{r}_i$ depends on the model parameters $\phi$. Using the product rule, the gradient of the expected loss in \Cref{eqn:small_obj} with respect to $\phi$ yields
    \begin{align*}
        \nabla_{\phi} \mc{L}_{\texttt{Small}}(\phi) \, |_{\phi = \phi_{\text{old}}} &= \frac{1}{G}\sum_{i=1}^G  \sum_{t=1}^N \mbb{E} \biggl[ \underbrace{\widetilde{A}_{i, t} \cdot \nabla_{\phi} \log \pi_{\phi}\left( o_{i,t} \, | \, q, o_{i, <t}\right)}_{\text{policy gradient}} +  \underbrace{\nabla_{\phi}\widetilde{r}_i(\phi) - \nabla_{\phi} \mathrm{mean}\left(\widetilde{\mathbf{r}}(\phi) \right)}_{\text{reward gradient from KD}}\biggr],
    \end{align*}
where 
\begin{align*}
    \nabla_{\phi}\widetilde{r}_i(\phi) = -\alpha \cdot \frac{1}{N} \sum_{t=1}^N \nabla_{\phi} \log \pi_{\phi}\left( o_{i,t} \, | \, q, o_{i, <t}\right).
\end{align*}
Notice that 
\begin{align}
\label{eqn:kd_term_zero}
    \mbb{E}_{o_i \sim \pi_{\phi}(\cdot | q)}\left[ \nabla_{\phi}\widetilde{r}_i(\phi)\right] &= -\alpha \cdot \frac{1}{N} \sum_{t=1}^N \mbb{E}_{o_i \sim \pi_{\phi}(\cdot | q)}\left[\nabla_{\phi} \log \pi_{\phi}\left( o_{i,t} \, | \, q, o_{i, <t}\right)\right] \\
    &= -\alpha \cdot \frac{1}{N} \sum_{t=1}^N \nabla_{\phi}\int \pi_{\phi}\left( o_{i,t} \, | \, q, o_{i, <t}\right) \tag{Tower Property} \\
    &= -\alpha \cdot \frac{1}{N} \sum_{t=1}^N \nabla_{\phi}1 \\
    &= 0.
\end{align}
Hence, the reward gradient from KD is zero in expectation, yielding the following remaining gradient:
\begin{align*}
    \nabla_{\phi} \mc{L}_{\texttt{Small}}(\phi) \, |_{\phi = \phi_{\text{old}}} &= \frac{1}{G}\sum_{i=1}^G  \sum_{t=1}^N \mbb{E} \biggl[ \widetilde{A}_{i, t} \cdot \nabla_{\phi} \log \pi_{\phi}\left( o_{i,t} \, | \, q, o_{i, <t}\right) \biggr].
\end{align*}
For simplicity in notation, let us denote 
\begin{align*}
    s_i \coloneqq \sum_{t=1}^N \nabla_{\phi} \log \pi_{\phi}\left( o_{i,t} \, | \, q, o_{i, <t}\right).
\end{align*}
Then, using the fact that $\widetilde{A}_{i, t} = \widetilde{A}_i = \widetilde{r}_i - \mathrm{mean}(\widetilde{\mathbf{r}})$, notice that
\begin{align*}
     \frac{1}{G} \sum_{i=1}^G \widetilde{A}_i \cdot s_i &= \frac{1}{G}\sum_{i=1}^G  \widetilde{r}_i \cdot s_i -  \frac{1}{G} \mathrm{mean}(\widetilde{\mathbf{r}}) \sum_{i=1}^G s_i \\
     &= \frac{1}{G}\sum_{i=1}^G  \widetilde{r}_i \cdot s_i - \frac{1}{G^2} \left(\sum_{j=1}^G \widetilde{r}_j \right) \left(\sum_{i=1}^G s_i \right).
\end{align*}
By taking the conditional expectation on $q$, we obtain
\begin{align*}
    \mbb{E}\left[ \frac{1}{G}\sum_{i=1}^G  \widetilde{r}_i \cdot s_i \, | \, q \right] - \mbb{E}\left[ \frac{1}{G^2} \left(\sum_{j=1}^G \widetilde{r}_j \right) \left(\sum_{i=1}^G s_i \right) \, | \, q \right] &= \mbb{E}[\widetilde{r}_i s_i \, | \, q] - \frac{1}{G^2}\sum_i^{G} \mbb{E}[\widetilde{r}_i s_i \, | \, q] + \frac{1}{G^2}\underbrace{\sum_{i \neq j}\mbb{E}[\widetilde{r}_j s_i \, | \, q]}_{=0} \\
    &= \left(\frac{G-1}{G}\right) \mbb{E}\left[\widetilde{r}_i s_i \, | \, q \right]
\end{align*}
Taking the average over $q$, we have
\begin{align}
\label{eqn:grpo_grad}
    \nabla_{\phi} \mc{L}_{\texttt{Small}}(\phi) = \left(\frac{G-1}{G}\right) \cdot \mbb{E}\left[\widetilde{r}_i \cdot  \sum_{t=1}^N \nabla_{\phi} \log \pi_{\phi}\left( o_{i,t} \, | \, q, o_{i, <t}\right)  \right].
\end{align}
Now we derive the true policy gradient by defining the reward objective:
\begin{align*}
    J(\phi) \coloneqq \mbb{E}_{q\sim P(Q), o_i\sim \pi_{\phi}(\cdot | q)} \left[ \widetilde{r}_{\phi}(q, o_i)\right],
\end{align*}
which yields
\begin{align*}
    \nabla_{\phi}J(\phi) &= \mbb{E} \left[ \widetilde{r}_{\phi}(q, o_i) \cdot \nabla_{\phi}\log \pi_{\phi}\left(o_i \, | \, q\right) \right] + \underbrace{\mbb{E}\left[\nabla_{\phi}\widetilde{r}_{\phi}(q, o_i) \right]}_{=0 \text{  (previously derived)}} \\
    &= \mbb{E} \left[ \widetilde{r}_{\phi}(q, o_i) \cdot \sum_{t=1}^N\nabla_{\phi}\log \pi_{\phi}\left(o_{i, t} \, | \, q, o_{i, <t}\right) \right].
\end{align*}
Then by multiplying the learning rate $\eta$ on both sides for the update rule:
\begin{align*}
    \eta \cdot \nabla_{\phi}J(\phi) &= \eta \cdot \mbb{E}\left[\widetilde{r}_i \cdot \sum_{t=1}^N \nabla_{\phi} \log \pi_{\phi}\left( o_{i,t} \, | \, q, o_{i, <t}\right)  \right] \\
    &= \underbrace{\eta \left(\frac{G}{G-1} \right)}_{= \eta_{\text{eff}}} \nabla_{\phi} \mc{L}_{\texttt{Small}}(\phi) \\ 
    &= \eta_{\text{eff}} \cdot\nabla_{\phi} \mc{L}_{\texttt{Small}}(\phi),
\end{align*}
which completes the proof.
\end{proof}

==> text/method_old.tex <==
\section{CoDistill-GRPO: An Efficient Co-Distillation Recipe for GRPO}
\label{sec:method}

\textcolor{red}{Ziteng: This section could be organized a bit better. I ould probably start by providing an overview of the algorithm including a step-by-step work through of the overall flow of CoDistill-GRPO including hinting with the large model, completing the rollout with the small model, downsampling, and then update the small model, and update the large model. I think now you have the content in Figure 2 and Algorithm 1. But I think given that there are so many components, it is still better if you can write out a walkthrough in English. Then you can say you break down each of the components in different subsections.
}


\textcolor{red}{Another note. Now in the subsections, the design choices and key algorithmic components are kind of mixed. It might be good to separate them and emphasize more on the key components. For example, omitting the regularizer is a design choice we made based on experimental resutls. But adding the KL term to the reward is a key algorithmic component. Another example, adding hints is a key algorithmic component to prompt higher-quality generations. And only adding hints in the first few iterations is a design choice based on stability of the training.}
In this section, we present 
each component of CoDistill-GRPO following the flowchart in \Cref{fig:hybrid_grpo}. Throughout this section, we use $\theta$ and $\phi$ to denote the parameters of the large and small models, respectively, and use $\pi_\theta$, $\pi_\phi$ to denote the corresponding policies. In \Cref{sec:small_grpo_obj}, we present the loss function for the small model $\mc{L}_{\texttt{Small}}(\phi)$ and in \Cref{sec:large_model_obj}, we present the loss function for the large model  $\mc{L}_{\texttt{Large}}(\theta)$. Then, in \Cref{sec:rejection}, we present the downsampling mechanism.
Lastly, in \Cref{sec:theory}, we present theoretical guarantees regarding the small model loss $\mc{L}_{\texttt{Small}}(\phi)$ and its use of the on-policy KD reward. We summarize CoDistill-GRPO and provide its pseudocode in \Cref{alg:algorithm}.



\begin{algorithm}[t!]
\caption{CoDistill-GRPO: Jointly Training Models via Co-Distillation}
\begin{algorithmic}[1]
\REQUIRE Initial small policy $\pi_\phi$; Initial large policy $\pi_\theta$; Prompt set $\mathcal{D}$; Batch size $B$;  Hyperparameter $\alpha$; Train steps $K$; Rollout sizes $M$ (before downsampling), $G$ (after downsampling); Hint size $T$; Hint steps $H$ 
\FOR{$k = 1, \ldots, K$}
    \STATE Sample a batch $\mathcal{D}_B$ from $\mathcal{D}$
    % \STATE Update the old policy model $\pi_{\theta_{old}} \leftarrow \pi_\theta$
\IF{$k \in [H]$}
    \STATE Sample hinted rollouts from large policy: $\{o_{i, 1:T}\}_{i=1}^M \sim \pi_\theta(\cdot|q)$ for each prompt $q \in \mathcal{D}_B$
    \STATE Complete rollouts with small policy: $\{o_{i, T+1:N}\}_{i=1}^M \sim \pi_\phi(\cdot | q, o_{i, 1:T})$ for each prompt $q \in \mathcal{D}_B$
\ELSE
    \STATE Sample rollouts with small policy: $\{o_{i, 1:N}\}_{i=1}^M \sim \pi_\phi(\cdot | q)$ for each prompt $q \in \mathcal{D}_B$
\ENDIF
    \STATE Compute rewards $\{r(o_i, q), \widetilde{r}(o_i, q)\}_{i=1}^M$ for every sampled response $o_i$ and prompt $q \in \mc{D}_B$
    \STATE Downsample using $\widetilde{r}$ as a scoring metric to obtain $\{r(o_i, q), \widetilde{r}(o_i, q)\}_{i=1}^G$
    \STATE Compute joint loss $\mc{L}(\theta, \phi) \coloneqq \mc{L}_{\texttt{Large}}(\theta) + \mc{L}_{\texttt{Small}}(\phi)$
    \STATE Take gradient $\nabla_{\theta, \phi}\mc{L}(\theta, \phi) = \nabla_{\theta}\mc{L}_{\texttt{Large}}(\theta) + \nabla_{\phi}\mc{L}_{\texttt{Small}}(\phi)$ and update policies $\pi_\theta$ and $\pi_\phi$
\ENDFOR
\RETURN Large policy $\pi_\theta$ and small policy $\pi_\phi$
\end{algorithmic}
\label{alg:algorithm}
\end{algorithm}



\subsection{GRPO Objective for the Small Model}
\label{sec:small_grpo_obj}

We begin with the GRPO objective function for the small model, $\mc{L}_{\texttt{Small}}(\phi)$. Following the flowchart in \Cref{fig:hybrid_grpo}, the large model generates an initial $T\geq 0$ tokens as a hint for which the small model completes, which are then used to update both models.  For simplicity, let us initially assume that $T = 0$, i.e., the small model generates the entire set of outputs from some model $\pi_{\phi_{\text{old}}}$. The objective $\mc{L}_{\texttt{Small}}(\phi)$ has a very similar structure to \Cref{eqn:grpo}, where the differences are highlighted in \textcolor{blue}{blue}:
\begin{align}
&\mathcal{L}_{\text{Small}}(\phi) = \mathbb{E}_{q \sim P(Q), \textcolor{black}{\{o_i\}_{i=1}^G \sim \pi_{\phi_{\text{old}}}(\cdot | q)}} \\
&\left[\frac{1}{G}\sum_{i=1}^G \frac{1}{N}\sum_{t=1}^{N}  \min \left\{ \frac{\pi_{\phi}(o_{i,t}|q, o_{i, <t})}{\pi_{\phi_{\text{old}}}(o_{i,t} | q, o_{i, <t})}  \textcolor{blue}{\widetilde{A}_{i,t}}, \text{clip}_{\epsilon}\left(\frac{\pi_{\phi}(o_{i,t}|q, o_{i, <t})}{\pi_{\phi_{\text{old}}}(o_{i,t} | q, o_{i, <t})}\right) \textcolor{blue}{\widetilde{A}_{i,t}} \right\}\right],
\label{eqn:small_obj}
\end{align}
where
\begin{align}
\label{eqn:small_reward}
     \widetilde{r}_i &\coloneqq \widetilde{r}(q, o_{i}) = \underbrace{r(q, o_{i})}_{\text{original reward}}  + \underbrace{\alpha \cdot \frac{1}{N}\sum_{t=1}^{N}\log\left(\frac{\pi_{\theta}(o_{i,t}|q, o_{i, <t})}{\pi_{\phi}(o_{i,t} | q, o_{i, <t})}\right)}_{\text{on-policy KD reward}}, \\
     \widetilde{A}_{i, t} &\coloneqq \widetilde{A}_i = \widetilde{r}_i - \mathrm{mean}\left(\widetilde{\mbf{r}} \right),
\end{align}
$\alpha > 0$ is a hyperparameter and $N > 0$ denotes the number of maximum completion tokens. 
The only difference lies in the rewards (and hence advantages): in addition to the original reward (e.g., accuracy for mathematical problems), the small model considers an additional reward inspired by on-policy KD \citep{agarwal2024onpolicy}. This additional reward incentivizes the small model to generate outputs that the large model would also generate, while penalizing those that the large model would not. This reward drives the probability distribution of the small model closer to that of the large model, achieving two goals: (i) improving the performance of the small model and (ii) promoting the use of the small model's rollouts to update the large model. Note that we also do not divide by the standard deviation for the advantages, following  \cite{liu2025understanding}. 
% Since generating multiple rollouts with the small model is computationally inexpensive compared to the large model, this approach can potentially save training time.


The derivation of the effective reward $\widetilde{r}_i$ is also intuitive: if we consider the GRPO objective in \Cref{eqn:grpo} as a ``reward maximization'' problem with a KL regularization term between the small and large model, then we have the following:
%\zs{Should this be an equality?}
\begin{align}
    \underset{\phi}{\mathrm{max}} \,\, &\mbb{E}_{q \sim P(Q)}  \left[ \mbb{E}_{o_i \sim \pi_{\phi}} \left[r(q, o_{i})\right] - \alpha \cdot  \mbb{D}_{\text{KL}}[\pi_{\phi}(\cdot | q) \| \pi_{\theta}(\cdot | q) ]  \right]\\
    = \underset{\phi}{\mathrm{max}} \,\,  &\mbb{E}_{q \sim P(Q), o_i \sim \pi_{\phi}} \biggl[r(q, o_{i}) -\alpha \cdot \log\left(\frac{\pi_{\phi}(o_{i}|q)}{\pi_{\theta}(o_{i} | q)}\right) \biggr].
\end{align}
Then, by averaging over all completion tokens, we obtain the effective reward in \Cref{eqn:small_reward} for each rollout. Note that we normalize by $N$ instead of the length $|o_i|$ to mitigate any potential length bias~\citep{liu2025understanding}.




\paragraph{Discussion.} There are a few design choices here that are worthy of discussion. First, we use a different unbiased estimates of the KL divergence than in \Cref{eqn:kl_div} for the reward computation, as we find that using the estimator in \Cref{eqn:kl_div} makes training unstable. Second, notice that instead of incorporating the on-policy KD term into the reward, we could have directly added it to the objective function as done in \Cref{eqn:grpo}. However, we find that incorporating the KD term into the effective reward generally yields better performance even for the same values of $\alpha$. Finally, we do not include a regularizer from a reference policy, i.e., we set $\beta = 0$ in \Cref{eqn:grpo}. Prior work has shown that omitting this term often leads to better performance~\citep{liu2025understanding, hu2025openreasonerzeroopensourceapproach}, and we also aim for the small model to deviate from its initialization so that it can achieve sufficient improvement through GRPO.


\textcolor{red}{I think what we are doing (considering both terms) is a natural and correct way to do this. So listing out the two cases makes it a bit confusing. It seems this is mainly to distinguish us from BREAD if I understanding correctly. I am not sure whether this is helping or just confusing the readers.}

Now, let us consider the case when $T>0$. In this case, the large model generates an initial hint with $T$ tokens. We have two options for importance sampling: (i) perform importance sampling on all tokens respectively as such:
\begin{align}
&\underbrace{
\sum_{t=1}^{T} 
\min \biggl(
  \frac{\pi_{\phi}(o_{i,t}\mid q, o_{i,<t})}{\pi_{\theta_{\text{old}}}(o_{i,t}\mid q, o_{i,<t})}
  \,\widetilde{A}_{i,t},
  \text{clip}_{\epsilon}\biggl(
    \frac{\pi_{\phi}(o_{i,t}\mid q, o_{i,<t})}{\pi_{\theta_{\text{old}}}(o_{i,t}\mid q, o_{i,<t})}
  \biggr)\widetilde{A}_{i,t}
\biggr)
}_{\text{importance sampling on initial tokens from large model}}
\\
&\quad\quad\quad\quad\quad\quad+
\underbrace{
\sum_{t=T+1}^{|o_i|}
\min \biggl(
  \frac{\pi_{\phi}(o_{i,t}\mid q, o_{i,<t})}{\pi_{\phi_{\text{old}}}(o_{i,t}\mid q, o_{i,<t})}
  \,\widetilde{A}_{i,t},
  \text{clip}_{\epsilon}\biggl(
    \frac{\pi_{\phi}(o_{i,t}\mid q, o_{i,<t})}{\pi_{\phi_{\text{old}}}(o_{i,t}\mid q, o_{i,<t})}
  \biggr)\widetilde{A}_{i,t}
\biggr)
}_{\text{importance sampling on completed tokens from small model}},
\label{eqn:small_sampling}
\end{align}
or (ii) ignore importance sampling on the hint tokens and perform importance sampling solely on those produced by the small model, which would amount to just using \Cref{eqn:small_sampling}. The second option is what is similarly used in the objective function of BREAD~\citep{zhang2025bread}.
However, we find that the second option generally makes training unstable, while the first option does not perform as well as treating these initial tokens as if they were generated by the small model. Hence, even for $T>0$, we use the objective in \Cref{eqn:small_obj}.
Furthermore, we also observe that providing these initial tokens as hints for all iterations leads to instability. We hypothesize that this occurs because the small model often fails to complete rollouts correctly, which produces large gradients and results in unstable training. For this reason, we provide hints only during the early iterations as a warm start for the small model.
% Taken together, these two design choices create a clear distinction between our algorithm and BREAD.



\subsection{GRPO Objective for the Large Model}
\label{sec:large_model_obj}

The GRPO objective for the large model $\mc{L}_{\texttt{Large}}(\theta)$ is straightforward: it must account for the fact that rollouts are generated by the small model $\pi_{\phi_{\text{old}}}$. We handle this by treating the problem as an off-policy RL problem and applying importance sampling with respect to the small model's token-probability distribution, which leads to the following objective:
\begin{align}
&\mathcal{L}_{\text{Large}}(\theta) = \mathbb{E}_{q \sim P(Q), \textcolor{blue}{\{o_i\}_{i=1}^G \sim \pi_{\phi_{\text{old}}}(\cdot | q)}} \\
&\left[\frac{1}{G}\sum_{i=1}^G \frac{1}{N}\sum_{t=1}^{N}  \min \left\{ \frac{\pi_{\theta}(o_{i,t}|q, o_{i, <t})}{\textcolor{blue}{\pi_{\phi_{\text{old}}}(o_{i,t} | q, o_{i, <t})}} \hat{A}_{i,t}, \text{clip}_{\epsilon}\left(\frac{\pi_{\theta}(o_{i,t}|q, o_{i, <t})}{\textcolor{blue}{\pi_{\phi_{\text{old}}}(o_{i,t} | q, o_{i, <t})}}\right) \hat{A}_{i,t} \right\} \right].
\label{eqn:large_obj}
\end{align}
\Cref{eqn:large_obj} has the same structure as the GRPO objective in \Cref{eqn:grpo}, but now accounts for the rollouts generated via the small model. Similar to \Cref{sec:small_grpo_obj}, we omit the regularizer with the reference model.





\subsection{Downsampling}
\label{sec:rejection}

The remaining point of discussion on the algorithmic aspects of CoDistill-GRPO is the downsampling block in \Cref{fig:hybrid_grpo}. The main idea is as follows: since all rollouts are generated using the more inexpensive small model, we can produce $M > G$ rollouts and then select a subset of $G$ rollouts that will likely lead to the most informative  updates. While one option is to select the top-$G$ rollouts with the highest rewards, \citet{xu2025rolloutsusefuldownsamplingrollouts} show that choosing the top and bottom $G/2$ rollouts yields the best performance. The intuition is straightforward: this  maximizes reward variance and exposes the model to both strong and weak trajectories. Consequently, we select the top and bottom $G/2$ rollouts using the effective reward in \Cref{eqn:small_reward} as the scoring metric. Using the effective reward with KD as the score is natural, since these selected rollouts are also used to update the large model.



\subsection{Theoretical Results}
\label{sec:theory}

Here, we present a couple of theoretical results regarding the small model loss $\mc{L}_{\texttt{Small}}(\phi)$. First, although the small model uses an effective reward that incorporates the on-policy KD term, we show that it still enjoys desirable statistical properties such as an unbiased gradient estimate.
\begin{lemma}
\label{lem:unbiased}
    Let $\eta > 0$ and $G>1$ denote the learning rate and group size, respectively. 
    Suppose that for each prompt $q \sim P(Q)$, the outputs are sampled on-policy $\{o_i\}_{i=1}^G \sim \pi_{\phi}(\cdot \, | \, q)$  
    and $\pi_\phi$ is continuously differentiable.
    If the policy $\pi_\phi$ is updated using the effective learning rate $\eta_{\text{eff}} \coloneqq \left(\frac{G}{G-1}\right) \cdot \eta$ with advantage estimates in \Cref{eqn:small_reward}, then the gradient of \Cref{eqn:small_obj} is an  unbiased estimate of the true policy gradient:
    \begin{align}
        \eta_{\text{eff}} \cdot \mbb{E}\left[\nabla_{\phi} \mc{L}_{\texttt{Small}}(\phi)\right] = \eta \cdot \nabla_{\phi} J(\phi),
    \end{align}
where $J(\phi) \coloneqq \mbb{E}_{q\sim P(Q), o_i\sim \pi_{\phi}(\cdot | q)} \left[ \widetilde{r}_{\phi}(q, o_i)\right]$ is the true reward objective.
\end{lemma}

Second, using \Cref{lem:unbiased}, we prove that the gradient of $\mc{L}_{\texttt{Small}}(\phi)$ can be decomposed into two terms: a direction towards the original reward and a direction towards the large model. This formally shows that when $\alpha > 0$, the effective reward drives the small model towards the large model, explaining why the effective reward improves small model performance beyond standard GRPO.


\begin{theorem}[Gradient Decomposition]
\label{thm:gradient}
    Let $\alpha >0$ and $N > 0$ denote the KD regularization parameter and number of maximum completion tokens, respectively. Under the same conditions as \Cref{lem:unbiased}, for each prompt $q \sim P(Q)$, the expected gradient of $\mc{L}_{\texttt{Small}}(\phi)$ admits the following decomposition:
    \begin{align*}
        \eta_{\text{eff}} \cdot \mbb{E}\left[\nabla_{\phi} \mc{L}_{\texttt{Small}}(\phi) \, | \, q \right] = \eta\cdot \underbrace{\nabla_{\phi} \mbb{E}_{o_i \sim \pi_{\phi}(\cdot | q)}\left[r(q, o_i)\right]}_{\text{direction towards original reward}} - \eta \cdot \frac{\alpha}{N} \underbrace{\nabla_{\phi} \mbb{D}_{\texttt{KL}}\left( \pi_{\phi}(\cdot | q) \| \pi_{\theta}(\cdot | q)\right)}_{\text{direction towards large model}}.
    \end{align*}
\end{theorem}
When $\alpha > 0$, the on-policy KD reward introduces an additional direction towards the large model, whereas with $\alpha = 0$ we would only have the direction towards maximizing the original reward. This is similar in spirit to \cite{kdrl}, but adapted for the effective reward setting and rigorously derived. All proofs are deferred to \Cref{sec:deferred_proofs}.
